Caging in Time: A Framework for Robust Object Manipulation under Uncertainties and Limited Robot Perception

Real-world object manipulation has been commonly challenged by physical uncertainties and perception limitations. Being an effective strategy, while caging configuration-based manipulation frameworks have successfully provided robust solutions, they are not broadly applicable due to their strict requirements on the availability of multiple robots, widely distributed contacts, or specific geometries of robots or objects. Building upon previous sensorless manipulation ideas and uncertainty handling approaches, this work proposes a novel framework termed Caging in Time to allow caging configurations to be formed even with one robot engaged in a task. This concept leverages the insight that while caging requires constraining the object's motion, only part of the cage actively contacts the object at any moment. As such, by strategically switching the end-effector configuration and collapsing it in time, we form a cage with its necessary portion active whenever needed. We instantiate our approach on challenging quasi-static and dynamic manipulation tasks, showing that Caging in Time can be achieved in general cage formulations including geometry-based and energy-based cages. With extensive experiments, we show robust and accurate manipulation, in an open-loop manner, without requiring detailed knowledge of the object geometry or physical properties, or real-time accurate feedback on the manipulation states. In addition to being an effective and robust open-loop manipulation solution, Caging in Time can be a supplementary strategy to other manipulation systems affected by uncertain or limited robot perception.

==> includes/problem_setup.tex <==
\section{Robust Planar Pushing}

Our caging-in-time theory is practically applied to a specific quasi-static planar pushing problem. This approach uses a single line pusher to guide an object along predefined trajectories. Our approach diverges from traditional planar pushing methods by eliminating the need for closed-loop control and additional sensory feedback. Instead, this method leverages the prediction and propagation of the potential configuration set, requiring only the object's initial position to facilitate task execution in an open-loop system. This technique is adaptable to a variety of settings, including different object shapes, trajectory types, and in-task disturbances.

In this task, the object is abstracted to a simple bounding circle with radius $r$ without other additional shape information. The configuration space and the object's workspace are equivalent as the same 2D plane. By expanding the potential configuration set $Q_t$ with the bounding circle's radius $r$, as depicted in Fig. \ref{fig:POA1} (left), we define the \textbf{Potential Object Area} $A_t$, noted as POA. This area ensures that no part of the object extends beyond this area, providing a reliable approximation of the object's potential coverage.

Our methodology, as illustrated in Fig. \ref{fig:cgtp2}, constructs a virtual cage around the object, which is set to directly trace the target trajectory, ensuring the object follows a similar path. While the object remains stationary in the world frame without external forces, its motion under the cage frame is predictable based on the cage's active movement. In the cage frame, the cage is static while the object becomes the dynamic element, in line with our caging-in-time concept.

The frame transformation process is formulated as follows. The configurations of both the object and the cage frame are described using homogeneous coordinates in the SE(2) space, with $3 \times 3$ transformation matrices for the object $q_t$ and the cage $c_t$. The configurations in the world frame at two consecutive timesteps are $q_t, q_{t+1}$ and $c_t, c_{t+1}$, respectively.

The object's configuration transformation in the cage frame is expressed as:

\begin{equation}
q_{t \_c}=c_t^{-1} q_t, \quad q_{t+1 \_c}=c_{t+1}^{-1} q_{t+1}
\end{equation}


The motion of the object in the world frame is given by $v_{t\_q}=q_t^{-1} q_{t+1}$, while the cage's motion in the world frame is represented as $u_{t\_c}=c_t^{-1} c_{t+1}$.

To ascertain the object's motion within the cage frame, we employ the following relationships:
\begin{equation}
\begin{aligned}
v_{t \_c}&=  q_{t \_c}^{-1} q_{t+1 \_c} \\
& =(q_t^{-1} c_t) (c_{t+1}^{-1} q_{t+1}) \\
& =q_t^{-1} u_{t \_c}^{-1} q_{t+1}
\end{aligned}
\label{eq:cageframe}
\end{equation}

 By applying Eq.\ref{eq:cageframe}, we can predict the POA at each timestep, enabling us to modify the cage walls to ensure that the object remains within the cage throughout. The prediction on the interaction is introduced in the next section. As a result, the object consistently follows the intended trajectory with an error margin defined by the cage's dimensions. This robust framework renders the planar pushing problem solvable under the caging-in-time paradigm.
